Matching-Logic-Based Understanding of Polynomial Functors and their Initial/Final Models

In this paper, we investigate how the initial models and the final models for the polynomial functors can be uniformly specified in matching logic.

==> eptcsdata.tex <==
\providecommand{\firstpage}{41}
\providecommand{\publicationstatus}{H. Cheval, L. Leu\c{s}tean, A. Sipo\c{s} (Eds.):\\ 7th Symposium on Working Formal Methods (FROM 2023)\\
EPTCS 389, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{https://dx.doi.org/10.4204/EPTCS.389.4}{10.4204/EPTCS.389.4}}
\pdfoutput=1

